Linear Block Coding for Efficient Beam Discovery in Millimeter Wave Communication Networks

The surge in mobile broadband data demands is expected to surpass the available spectrum capacity below 6 GHz. This expectation has prompted the exploration of millimeter wave (mm-wave) frequency bands as a candidate technology for next generation wireless networks. However, numerous challenges to deploying mm-wave communication systems, including channel estimation, need to be met before practical deployments are possible. This work addresses the mm-wave channel estimation problem and treats it as a beam discovery problem in which locating beams with strong path reflectors is analogous to locating errors in linear block codes. We show that a significantly small number of measurements (compared to the original dimensions of the channel matrix) is sufficient to reliably estimate the channel. We also show that this can be achieved using a simple and energy-efficient transceiver architecture.

==> Analogy.tex <==
Channel estimation in mm-wave wireless channels have been shown to be sparse in nature.
Sparsity in this context refers to the availability of only few scattering clusters where each cluster has a small range of AoDs and AoAs at the TX and RX, respectively, such that individual reflectors among each cluster cannot be resolved.
Hence, the channel estimation problem is to identify the path gains associated with each cluster along with their AoDs and AoAs.
Ultimately, the TX aims is to identify the angles in which paths to its intended receiver exists and the gains of those paths to adjust the transmission power and rate.
Similarly, the RX aims to identify the angles at which its intended data stream(s) will arrive.
The difficulty arises because there are so many directions in which the TX and RX can focus on. In fact, there are as many directions at the TX and RX as their number of respective antennas which is large.
Hence, channel estimation using an exhaustive search would require a huge overhead that renders it practically impossible.

The idea of channel coding is to introduce some redundant parity bits for every transmitted information sequence where each parity forms some special combination of information bits such that the generated codewords are as far as possible in the Hamming distance sense.
Typically, for all codes that can correct up to $e_n$ bits in error, a good code is the one that can add as few parity bits as possible. Combine that with the fact that error syndrome decoding is performed using syndromes $\mathbf{s}$ of length $n{-}k$, the same number of parity bits, we can view the error syndrome as a diagnosis of an error pattern $\mathbf{e}$. Hence, elements of $\mathbf{s}$ can be thought of as a series of tests that lead to a perfect diagnosis of a correctable $\mathbf{e}$.

To simplify the analogy, we are going to present a toy problem with idealistic assumptions as follows:
Consider the communication link between a TX with a single antenna $n_t = 1$ and a receiver with $n_r$ antennas. Therefore the channel $\mathbf{h}$ is $(n_r {\times} 1)$ vector and its corresponding angular (virtual) channel $\mathbf{h}^a$ is a vector of the same size and can be derived using the DFT matrices $\mathbf{U_t}$ and $\mathbf{U_r}$ as $\mathbf{h}^a = \mathbf{U_r}^*\: \mathbf{h} \: \mathbf{U_t}$. 
%whose columns are the steering vectors of uniform linear arrays (ULA) of the TX and RX, respectively.
Assume that each cluster contains only one path with fixed path gain $a = 1$.
Further, lets assume perfect sparsity such that AoAs and AoDs are along the directions defined in the DFT matrices \cite{ChEstScniter14}. i.e. each path will only contribute to one angular bin.
Finally, lets also neglect the channel noise.

Hence, we get a channel vector of the form
\begin{equation}
\mathbf{h}^a = 
 \begin{pmatrix}
  h^a_0 \\
  h^a_1 \\
  \vdots\\
  h^a_{n_r-1}
 \end{pmatrix} 
\end{equation}
where $h^a_i \in \{0,1\}$. Also let the number of paths $L$, (i.e. number of non-zero elements in $\mathbf{h}^a$) be such that $L \leq e_n$ where $e_n$ is the maximum number of correctable bit errors of an $(n,k,d)$ code $C$. If the transmitter sends pilot symbols of the form $x = 1$, then the received vector $\mathbf{y}$ can be calulcated as
\begin{align}
\mathbf{y}   &=  \mathbf{h} x   =  \mathbf{h}
\end{align}
%\mathbf{y}^a &=  \mathbf{U_r}^* \: \mathbf{h} x \\
%\mathbf{y}^a &=  \mathbf{h}^a 
Now we can think of $\mathbf{h}^a$ as a received sequence with just a few non-zero components and our aim is to identify their positions. We consider these non-zero components to be anomalies to a normally all-zero angular channel.
Hence, the goal of identifying these positions is analogous to finding the most likely error pattern in channel coding.

\subsection{How to estimate the channel?}

At this point, we would like to proceed with channel estimation using the error syndrome decoding analogy as follows:
First we need to find the channel syndrome $\mathbf{h}_s$ similar to equation (\ref{eq:syndromeECC}) as follows
\begin{equation}
\mathbf{h}_s^T = \mathbf{h}^T . \mathbf{H}^T \Longrightarrow \mathbf{h}_s = \mathbf{H} . \mathbf{h}
\end{equation}
where $\mathbf{H}$ is the parity check matrix of an $(n,k,d)$ error correcting code $C$ with $e_n {=} L$ and $n {=} n_r$.

In practice, the process of obtaining $\mathbf{h}_s$ involves channel measurements such that each component ${h_s}_i$ of $\mathbf{h}_s$ is a separate measurement and can be found using
\begin{equation}
{h_s}_i = \mathbf{w}_i^T . \mathbf{h}
\end{equation}
where $\mathbf{w}_i$ is a receive beamforming vector of size $n_r {\times} 1$.
The design of each $\mathbf{w}_i \; \forall i \in \{1,2,\dots,n{-}k\}$ is based on the structure of the rows of $\mathbf{H}$. Let $[h_{i,j}]$ be the component along the $i^{th}$ row and $j^{th}$ column of $\mathbf{H}$.
Therefore, $\mathbf{w}_i$ is designed based on the $i^{th}$ row of $\mathbf{H}$, such that $\mathbf{w}_i$ combines the received $j^{th}$ channel components for all $[h_{i,j}] = 1$.

\subsection{Design of receive combining vectors}
The design of the receive combining vectors remains an important aspect of this work.
As an initial step towards obtaining proper receive combining vectors we consider the linear summation of individual analog beamformers of specific directions.
Let $\alpha_n$ be the weights of each antenna element in the antenna array and
let $y(\phi)$ be the received signal at angle $\phi$ after receive combining. Then
\begin{equation}
y(\phi) = \sum_{n=0}^{n_r-1} \alpha_n e^{-j2\pi n \Delta_r cos(\phi)}
\end{equation}
So, $\mathbf{\alpha}$, the receive analog combining vector, can be designed such that maximum gain can be observed at angle $\phi$ by setting its components as $\alpha_n = e^{j2\pi n \Delta_r cos(\phi)}$.

Now suppose that we extend this concept to multiple directions, e.g. $\phi_1$ and $\phi_2$, and let $\alpha_n = e^{j2\pi n \Delta_r cos(\phi_1)} + e^{j2\pi n \Delta_r cos(\phi_2)}$.
Hence, the received signal after receive combining will be
\begin{align}
y(\phi) &= \sum_{n=0}^{n_r-1} \big[e^{j2\pi n \Delta_r cos(\phi_1)} + e^{j2\pi n \Delta_r cos(\phi_2)}\big] . e^{-j2\pi n \Delta_r cos(\phi)}\nonumber \\
y(\phi) &= \sum_{n=0}^{n_r-1} e^{j2\pi n \Delta_r (cos(\phi_1)-cos(\phi))}
         + \sum_{n=0}^{n_r-1} e^{j2\pi n \Delta_r (cos(\phi_2)-cos(\phi))} \label{eq:RxCombineLinear}
\end{align}
Let $\phi_1$ and $\phi_2$ be such that $cos(\phi_1) = \frac{k_1}{n_r}$ and $cos(\phi_2) = \frac{k_2}{n_r}$ where $k_1 , k_2 \in \{0,1,\dots,n_r{-}1\}$ and $k_1 \neq k_2$, such that these angles are at the center of receive bins of the angular channel.
Suppose that $\phi = \phi_1$. Hence we can find the first summation of equation (\ref{eq:RxCombineLinear}) to give the same result of analog beamforming at $\phi = \phi_1$, while the second summation can be shown to be zero (\cite{•} or provide proof).
In other words, the choices of $\phi_1$ and $\phi_2$ are such that the steering vectors of those directions are orthogonal. In fact, those steering vectors are among the basis vectors of  the DFT matrix $\mathbf{U_r}$.

This method of designing the receive beamforming vectors $\mathbf{w}_i$ is ideal under the perfect sparsity assumption invoked in our toy problem where AoDs are along the directions defined in $\mathbf{U_r}$. However, linearly combining individual receive beamformers might yield undesirable performance for general AoDs. Specifically, the maximum gains of new beamformers are not exactly at the maximum directions of the individual directions, moreover, the side lobes have higher gains which is undesirable as well. See Fig. \ref{fig:RxBeamformingLinearCombining} for an example of linearly combining two different direction with $n_r = 7, k_1 = 0, k_2 =1$

\begin{figure}[t]
\centering
\includegraphics[width=0.5\linewidth]{Figs/RXBeamformingLinearCombining.eps}
\caption{Example of Receive beamforming using linear combining}
\label{fig:RxBeamformingLinearCombining} 
\end{figure}


\subsection{Example}

For more elaboration, we build on the previous toy problem and provide a numeric example as follows.
Let the number of receive antennas be $n_r = 7$ and the number of paths be just one (i.e. $L {=} 1$) with path gain $a{=}1$.
Thus, the channel contains only one strong component in the angular domain while the rest are zeros.

To solve the problem we need to choose a LBC with $n = 7$ and $L = e_n = 1$ (actually we just need $n \geq n_r$ and $e_n \geq L$). Therefore, the $(7,4,3)$ Hamming code is a suitable choice. Its parity check matrix can be given by
\begin{equation}
\mathbf{H} = 
  \begin{pmatrix}
  1 & 1 & 0 & 1 & 1 & 0 & 0 \\
  1 & 0 & 1 & 1 & 0 & 1 & 0 \\
  0 & 1 & 1 & 1 & 0 & 0 & 1 \\
  \end{pmatrix}  
\end{equation}

The channel syndrome is given by
\begin{equation}
\mathbf{h}_s = 
  \begin{pmatrix}
  {h_s}_0  \\
  {h_s}_1  \\
  {h_s}_2  \\
  \end{pmatrix}
  =
  \begin{pmatrix}
  \mathbf{w}_0^H . \mathbf{h}\\
  \mathbf{w}_1^H . \mathbf{h}\\
  \mathbf{w}_2^H . \mathbf{h}\\
  \end{pmatrix}  
\end{equation}
Consider the first receive beamforming vector $\mathbf{w}_1$. According to $\mathbf{H}$, we should design it such that it combines directions $1,2,4,5$, i.e. $\mathbf{w}_1 = \sum_i \mathbf{\alpha_i}$ where $i \in \{1,2,4,5\}$,
\begin{equation}
\mathbf{\alpha_i} = 
  \begin{pmatrix}
  1    							    	  \\
  e^{-j2\pi   \Delta_r cos(\phi_i)}  	  \\
  e^{-j2\pi 2 \Delta_r cos(\phi_i)}  	  \\
  \vdots								  \\
  e^{-j2\pi (n_r-1) \Delta_r cos(\phi_i)}  \\
  \end{pmatrix},
\end{equation}
and $cos(\phi_i) {=} \frac{i-1}{n_r}$.
Similarly, we design $\mathbf{w}_1$ and $\mathbf{w}_2$.
At this point, we can just construct a look-up table of all possible channel syndromes and their corresponding channels (i.e. $\mathbf{h}_s \Longrightarrow \mathbf{h}^a$) just like the error syndrome decoding in ECC.
For example, if AoA angular cosine $cos(\phi) {=} \frac{5}{7}$, then,
\begin{equation}
\mathbf{h}_s = 
  \begin{pmatrix}
  \sqrt{7} \times 1  \\
  0       \\
  \sqrt{7} \times 1 \\
  \end{pmatrix}
\Longrightarrow
\mathbf{h}^a = 
  \begin{pmatrix}
  0  \\
  0  \\
  0  \\
  0  \\  
  0  \\
  1  \\
  0
  \end{pmatrix}
\end{equation}
where $\sqrt{7} \times 1$ is the receive antenna gain $\times$ the path gain.

The toy problem we considered is actually an AoA estimation problem since $a = 1$ is assumed known.
Naturally, there exists more paths $L$ with unknown gains $a_l \in \mathbb{C}$, multiple antennas at the TX and RX. Also AoAs and AoDs are not strictly at the center of each TX and RX bin of the angular channel.
Next we present the system model for the general problem.


==> LBC.tex <==
In this work, we focus on linear block error correction codes.
Let $\boldsymbol{x_i}$ denote binary information sequence $i$ where $\boldsymbol{x_i}$ is a row vector of length $k$ $ \: \forall i$. Thus, there exists a total number of $2^k$ possible information sequences.
An $(n,k,d)$ block code $C$ is completely defined by $M = 2^k$ binary codeword (CW) sequences of length $n$ where each information sequence $\boldsymbol{x_i}$ is mapped to a CW $\boldsymbol{c_i}$.
Let $\oplus$ denote the bit-wise module-2 sum operation.
If $\boldsymbol{c_i}, \boldsymbol{c_j} \in C$ then $C$ is a binary linear block code if and only if $\boldsymbol{c_t} = \boldsymbol{c_i} \oplus \boldsymbol{c_j}$ is also a CW in $C$.
In fact, the CWs of $C$ form a $k$-dimensional subspace of the $n-$dimensional vector space $V^{n}$ formed by all $n-$tuples over the Galois (finite) fields $GF(2)$.

The error correction capability of an LBC code $C$ is characterized by its minimum distance $d$ where the number of correctable errors $e_n$ is be given by
\[
  e_n =\begin{cases}
               \frac{d-1}{2}, & d \text{ is odd}\\
               \frac{d-2}{2}, & d \text{ is even}
            \end{cases}
\]

\subsection{Generator and Parity Check Matrices}
An LBC code can be completely defined by its generator matrix $\boldsymbol{G}$ and parity check matrix $\boldsymbol{H}$.
An $(n,k,d)$ code $C$ is a $k-$dimensional subspace of a vector space $V^n$, hence, we can find a set of $k$ linearly independent CWs $\boldsymbol{g_0}, \boldsymbol{g_1}, \dots , \boldsymbol{g_{k-1}}$ such that any CW $\boldsymbol{c}  \in C$ can be written as a linear combination of these $k$ CWs. i.e.
\begin{equation}
\boldsymbol{c} = x_0 \boldsymbol{g_0} + x_1 \boldsymbol{g_1} + \dots + x_{k-1} \boldsymbol{g_{k-1}},
\end{equation}
where $x_i \in \{0,1\} \forall i \in 0,\dots,k{-}1$.

The structure of the generator matrix $G$ of code $C$ can be quite general, nevertheless, we can always find an equivalent systematic code in which every CW starts with a replica of the information sequence itself followed by $n-k$ parity bits. A necessary and sufficient condition for the code to be systematic is that its generator matrix be in the form
\begin{align}
\boldsymbol{G} &= [\boldsymbol{I_k} \: | \: \boldsymbol{P}] \nonumber \\
  &= 
  \begin{pmatrix}[cccc|cccc]
  1 & 0 & \cdots & 0  & p_{0,k} &p_{0,k+1} &\cdots &p_{0,n} \\
  0 & 1 & \cdots & 0  & p_{1,k} &p_{1,k+1} &\cdots &p_{1,n} \\
  \vdots  & \vdots  & \ddots & \vdots   &   \vdots  & \vdots  & \ddots & \vdots \\
  0 & 0 & \cdots & 1 & p_{k-1,k} &p_{k-1,k+1} &\cdots &p_{k-1,n} 
 \end{pmatrix}  
\end{align}

CWs are arranged as row vectors of size $1 \times n$ while the information sequences, $\boldsymbol{x_i}$'s, are $1 \times k$ row vectors.
Therefore, we can write the CWs $\boldsymbol{c}$ as
\begin{equation}
\boldsymbol{c} = \boldsymbol{x}\boldsymbol{G}
\end{equation}


Associated with every code $C$ is a dual (orthogonal) $(n,n-k)$ code denoted by $C^\perp$ such that $C^\perp$ spans the complementary $(n{-}k)$ dimensional subspace of the vector space $V^n$ in which the CWs of $C$ live. Let the generator matrix of $C^\perp$ be $\boldsymbol{H}$.
Therefore, it follows that the CWs of $C$ and $C^\perp$ are orthogonal to each other. Hence,
\begin{equation}
\boldsymbol{C}\boldsymbol{H}^T = 0
\end{equation}
The matrix $\boldsymbol{H}$ is called the parity check matrix of the code $C$ and is given by
\begin{align}
\boldsymbol{H} &= [\boldsymbol{P}^T \: | \: \boldsymbol{I_{n-k}}] 
\nonumber \\
	&=
  \begin{pmatrix}[cccc|cccc]
  p_{0,k} & p_{1,k} & \cdots & p_{k-1,k}  & 1 &0 &\cdots &0 \\
  p_{0,k+1} & p_{1,k+1} & \cdots & p_{k-1,k+1}  & 0 &1 &\cdots &0 \\
  \vdots    & \vdots    & \ddots & \vdots       &   \vdots  & \vdots  & \ddots & \vdots \\
  p_{0,n}   & p_{1,n}   & \cdots & p_{k-1,n}    & 0 &0 &\cdots &1 
 \end{pmatrix}
\end{align}

\subsection{Decoding}

A received sequence can be given by $\boldsymbol{r} = \boldsymbol{c}  + \boldsymbol{e}$ where $\boldsymbol{c}$ is the transmitted CW and $\boldsymbol{e}$ is the error pattern added over the noisy channel.
Decoding the received sequence boils down to figuring out the most likely error pattern, $\boldsymbol{\hat{e}}$, that occurred over the channel. For binary sequences, an error sequence has a value $1$ at the positions where errors have occurred. Subtracting $\boldsymbol{\hat{e}}$ from $\boldsymbol{r}$ yields the most probable transmitted CW, i.e., $\boldsymbol{\hat{c}} = \boldsymbol{r} - \boldsymbol{\hat{e}}$.
%Decoding errors, i.e., $\boldsymbol{\hat{c}} \neq \boldsymbol{c}$ can still happen for uncorrectable error patterns.
Basically, decoding a received sequence $\boldsymbol{r}$ entails finding its closest CW in the Hamming Distance sense.
Let $d(\boldsymbol{r},\boldsymbol{c_i})$ denote the hamming distance between the sequences $\boldsymbol{r}$ and $\boldsymbol{c_i}$.
Computing $d(\boldsymbol{r},\boldsymbol{c_i}) \: \forall i$ can be prohibitively complex, hence, more systematic ways that exploit the nice characteristics of linear block codes are used. 

When the sequence $\boldsymbol{r}$ is received, the receiver computes the $1 {\times} (n{-}k)$ error syndrome vector $\boldsymbol{s}$ as follows
\begin{align}
\boldsymbol{s} &= \boldsymbol{r} \boldsymbol{H}^T \label{eq:syndromeECC} \\ 
           &= (\boldsymbol{c} + \boldsymbol{e}) \boldsymbol{H}^T = \boldsymbol{c} \boldsymbol{H}^T + \boldsymbol{e} \boldsymbol{H}^T\\
           &= \boldsymbol{e} \boldsymbol{H}^T  \label{eq:SyndromeCodeOrthog}
\end{align}
where equation (\ref{eq:SyndromeCodeOrthog}) follows from orthogonality of $\boldsymbol{c}$ and $\boldsymbol{H}$.

The error syndrome $\boldsymbol{s}$ is a sufficient statistic for the decoding problem. Thus, an error syndrome uniquely identifies a correctable error pattern, (i.e., $\boldsymbol{s} \Rightarrow \boldsymbol{e})$.
Therefore, upon calculating $\boldsymbol{s}$, we can identify which error pattern-most likely-occurred and hence we can find $\boldsymbol{\hat{c}}$. The mapping from $\boldsymbol{s}$ to $\boldsymbol{e}$ is usually done using using a look-up table called the \textit{standard array}. This method is only reasonable when the distinct number of error syndromes, $2^{n-k}$, is small.
Other decoding methods that do not require a look-up table can be possible for some codes, e.g., BCH and Reed-Solomon codes.
